Less is More: Fairness in Wide-Area Proof-of-Work Blockchain Networks

Blockchain is rapidly emerging as an important class of network application, with a unique set of trust, security and transparency properties. In a blockchain system, participants record and update the `server-side' state of an application as blocks of a replicated, immutable ledger using a consensus protocol over the Internet. Mining blocks has become lucrative in recent years; e.g., a miner receives over USD 200,000 per mined block in Bitcoin today. A key factor affecting mining rewards, is the latency of broadcasting blocks over the network. In this paper, we consider the problem of topology design for optimizing mining rewards in a wide-area blockchain network that uses a Proof-of-Work protocol for consensus. Contrary to general wisdom that a faster network is always better for miners, we show a counter intuitive result where a slower network is actually beneficial to some miners. This is because competing miners must choose neighbors that not only decrease their own latency to others, but also ensure that the latency between other miners do not decrease because of itself. We formalize this problem, and provide both theoretical analysis and experimental results to support our claim.

==> Figures/evaluation.tex <==
\section{Evaluation}
\label{s: evaluation}
In this section we present experimental evaluation to highlight reward bias due to clustering discussed in Section~\ref{s: analysis}, in real-world settings.
% including bitcoin mining, broadcasting and the longest chain strategy. 
% Then we conduct experiments with the delay collected in reality and present the bias in the current network.
We then present candidate protocols that miners can adopt in order to alleviate the bias and increase their profits. 
% characterize the network connectivity that affects the bias and give some advice to the miners to get the best of their profits.

\subsection{Simulation Model}
\label{s: eval model}
We conduct our experiments on OMNeT++ 5.6.2, an event driven simulator~\cite{varga2008overview}, by implementing a detailed model based on the Bitcoin protocol. 
There are 246 miners in our simulation, with each miner mining blocks, broadcasting messages and maintaining a local replica of the blockchain in a completely decentralized fashion. 
% in a bitcoin network, with the similar strategy to mine the block, broadcast message and keep the longest blockchain at each node locally.
Note that this model we have used in the simulations, is significantly different from the simple analytical model discussed in Section~\ref{s: sysmodel}.  

\smallskip
\noindent
\textbf{Mining.}
We apply Bitcoin's mining and broadcasting strategy in our simulation.
At the start of the simulation, all the nodes mine the block on top of the genesis block.
To simulate mining, each miner has an independent random timer that expires according to an exponential distribution of a certain rate.
We use the same rate for all miners, to model uniform hash power across all miners. 
%  get an expected mining time from the exponential distribution based on nodes' hash power and the network's mining difficulty.
When a miner's timer expires, it generates a block on top of the block with the greatest height on its blockchain, and broadcasts it immediately to its connected neighbors.\footnote{Ties are broken as explained in Section~\ref{s: background}.} 
%  After waiting for the expected mining time, a node mines the block and broadcast this immediately to its connected neighbors.
When a miner is waiting for its timer to expire, if it receives a new block that extends its current longest chain, it updates it local blockchain and resets the timer to mine on top of the new received block.
%. The previous mining is invalid and this node restarts the mining work based on the newly received longest block.

\smallskip
\noindent
\textbf{Block broadcast.}
Miners receive and generate messages of different types, each of which causes the state of the miner to be updated as follows. 
% When a miner receives a block from a neighbor, it immediately relays the block to all neighbors except the one from which it received the block. 
%  relay any block they received to all their neighbors except the one from which they received it. 
% communicate their longest chain by broadcasting the latest block they received to their neighbors.
% When the neighbors receive the newly mined blocks, they compare the block's height with their longest chain and validate it if its parent block is in their block chain.
\begin{itemize}
\item[*] Blocks are messages that have an identifier and a pointer to the parent block's identifier.
We do not include any transactions in a block message; nor do we model bandwidth limitations in the network. 
When a miner receives a block message, it first validates the block by verifying it points to a valid parent block in its blockchain.
If the received block is valid and extends the longest chain in the blockchain by one, the miner adds the block in to its blockchain. 
%  is longer and valid, add this block into the block chain and accept this one as the longest chain. 
It then resets its exponential timer to mine a new block over the latest received block.
% previous mining task, generate a new expected mining time and start to mine based on the newly received block.
We set a duration of 1 ms at each miner for this validation operation. 
Upon validation, the miner immediately sends out the block message to all of its neighbors except the one it received it from. 
\item[*] A miner may also receive a block message, whose parent block is unavailable at the miner's local blockchain replica. 
In this case, the miner sends a `require' message back to the sender of the block requesting to also send the parent block. 
The received block is meanwhile stored within an orphan block list at the miner. 
We set a duration of 1 ms at each miner for this operation as before. 
When a miner receives a require message, it sends back the requested block as a `response' message.
% If the received one is longer but not valid, send a require message back the require its parent block and store the received one into orphan block list. 
In case the response block message received to the require message is also such that its parent block is unavailable, a second require message is sent. 
% Send a require message back again if the received parent block is still invalid. 
This process continues until all blocks from the genesis to the first received block are available. 
% So on and so forth until get the full path from the new received block to the genesis block, add them to the block chain and accept it as the longest chain.
\item[*] If a miner receives a block that is not part of the longest chain, it adds the block in to the blockchain, and does not relay the block to any of the neighbors. 
% If the received one is not longer and valid, add it into the block chain following its parent block.
% \item[*]If the received one is not longer and not valid, store it into orphan block list.
\end{itemize}

% The require message and its response message can help nodes to communicate their block chain until the requirer gets the complete block chain list by filling all the missing blocks from the genesis block to the newly received block.
% Each time nodes received the require block message, they check whether their parent block is inside the block chain to valid the require block message. 
% If the required block is invalid, keep requiring the parent of the required block. Otherwise, add the block all its child blocks in the orphan list into the block chain.
% Under such strategy, nodes keep updating their longest chain with all the reachable information from their neighbors and mining mining based on their longest chain,

\smallskip 
\noindent
\textbf{Reward.}
Miners earn rewards by mining blocks that get included in the longest chain.
% If multiple miners mine blocks with the same height, only one miner can get the bitcoin reward whose mined block is accepted by the whole network.
% So it's a competition between miners, not only to mine the block quicker than the others but also to broadcast the mined block to the total network quicker to let the others accept this block earlier and mine based on this block.
% Miners try their best the maximize the mined blocks in the longest chain, 
We measure reward by computing the percentage fraction of blocks mined by a miner that is included in the longest chain, i.e., the $F_v$ values for each miner $v$ as defined in Equation~\eqref{eq: Fv define}. 
% in order to measure the nodes' performance in different topologies, we care about the number of mined blocks in the accepted longest chain.
While it is likely that the blockchain replicas at different miners are not 100\% consistent with each other, it is typically the case that the longest chain except for the last few blocks is consistent across miners. 
% For the most network environment settings, the propagation delay are not long enough so that nodes can synchronize their longest chain except the the last several blocks.
So we discard the last 100 blocks in the longest chain, and collect the percentage of valid blocks among the remaining blocks in the longest chain for each miner.
Each experiment is run for a sufficient duration that more than 100,000 blocks are present in the longest chain at the end of the simulation. 
This ensures there are at least a 100 blocks mined per miner within the longest chain. 
% During our simulation, we run a lone enough time to enable more than 100,000 blocks in the longest chain so that most nodes can mine hundreds blocks in the longest chain.
For each network topology, we run 10 independent simulations to gather confidence in the reported results. 
% We also run each topology for 10 times to get a lower influence from randomness.

\smallskip
\noindent
{\bf Network model.} 
We consider 246 miners distributed across cities around the world. 
There are 94 miners from Europe, 83 from North America, 37 from Asia, 12 from South America, 11 from Africa and 9 from Australia.
This geographical distribution of miners is representative of the Bitcoin network's miner distribution~\cite{bitnodes} that has a majority of nodes at Europe and North America. % , so we apply the corresponding 246 nodes 
The propagation delay of messages between any two miners is set according to the global ping statistics dataset collected on July 19th \& 20th, 2020 from WonderNetwork~\cite{wondernetwork}.
We take half of the average measured round-trip times as the propagation delay between any two miners that are neighbors in a topology. 
%if they are the neighbors that have the direct connection in the topology to measure.
% There are 246 active servers, 94 servers among them from Europe, 83 from North America, 37 from Asia, 12 from South America, 11 from Africa and 9 from Australia.
% The continent distribution is close to the Bitcoin network's distribution that has the majority nodes at Europe and North America, so we apply the corresponding 246 nodes 
We consider all messages to be small in size, and do not model bandwidth at the miners. 
% with the region and propagation delay information.
We have set the delay in processing messages to be a low value of 1 ms, as in reality miners (e.g., in Bitcoin) have a significant compute power available to them.
The primary delay bottlenecks in our experiments are therefore the mining time and propagation delay. 
%  Consider that miners shall mine with high hash power in reality, which can quickly process the messages, so we set the process delay to be 1ms which is lower than the propagation delay and mining time.


\subsection{Results}

\subsubsection{Validate the theoretical model}
There are some differences between the theoretical model and Omnet++ model.
For example, Omnet++ processes the mining task continuously without waiting for the next round. 
So we first construct the network based on the theoretical to proof its generality.
We set a 20-node network. Each node has an expectation of 6000 ms average mining time with link delay from 0 ms to 400ms.

\begin{figure*}[!tbp]
  \centering
  \subfigure[]{\includegraphics[width=0.5\textwidth]{Figures/oneClusterChangeDelay.png}\label{fig:theoreticalModel1}}
~~
  \subfigure[]{\includegraphics[width=0.5\textwidth]{Figures/twoClusterChangeSize.png}\label{fig:theoreticalModel2}}
  \caption{TO DO.
  }
  \label{fig:theoreticalModel}
\end{figure*}

Figure~\ref{fig:theoreticalModel1} shows that nodes can efficiently communicate their blocks with a low delay environment, but such efficiency decreases with a higher delay.

Based on the fork rate results, we now evaluate the 2-cluster network.
With the same 20 nodes, we split them into 2 clusters, cluster A and B.
Nodes in the same cluster have a 30ms delay but have a 360 ms delay to the other cluster.
Then we adjust the size of cluster B to increase from 1 node until 11 nodes, while the size of cluster A decreases from 19 to 9.

In Figure~\ref{fig:theoreticalModel2} we pick 2 random nodes $A_i$ and $B_i$. While node $A_i$ is the node in cluster A during all our experiments and nodes $B_i$ is the node always in cluster B.
We record their percentage of valid blocks in the longest chain to learn their harvest with the change of their belonging cluster's size.
Node $A_i$  starts around 5\% in a 19-node network where the cluster A occupy most of the blockchain and distribute to 19 its nodes.
Nodes in cluster A gets more percentage around size 14 and then decreases to meet node $B_i$ with the same size of 10 nodes.
Node $B_i$ gets a higher percentage and a greater slope with the increasing of cluster B's size. 
The large size cluster can easily defeat the small size cluster and get a higher percentage of blocks in the longest chain.
Such advantage brings a benefit in the mining competition to every node.
But the maximum benefit appears at 14-node cluster in our 20-node network.
After that, the large cluster can hardly plunder a larger cake but more miners in the cluster share the cake.

The difference in mining schedule and message exchange brings a higher fork rates in the bitcoin network model.
However, the results in the experiments follows the theoretical model's conclusions.

\subsubsection{Natural clustering due to miner locations} 
The simple theoretical model liked network proofs the results. 
Since the network in reality is much larger and complicated, we apply the global ping statistics from WonderNetwork to set a 246-node network with random connection topology and complete graph topology.
Similar to the topology followed by the current Bitcoin network,  the random topology randomly pick a fixed number of neighbors for each node.
Limited by the size of the network, we set a lower neighbor degree at 6 rather than 8.
Nodes build the connections to their neighbors and accept the connections from the others.
The complete graph topology is to connect nodes by a complete graph so that all the nodes have a direct connection to every other node.

\begin{figure*}[!tbp]
  \centering
  \subfigure[]{\includegraphics[width=1\textwidth]{Figures/randomandcomplete.png}\label{fig:randomandcom}}
  \caption{TO DO.
  }
  \label{fig:Naturall}
\end{figure*}

Figure~\ref{fig:randomandcom} shows that the Europe and North America are the dominant clusters.
In the 246 node network, there's a fair state around 0.4\% for the 246 nodes with uniform hash power.
However, modes European and North American nodes get a greater percentile than the fair state while the others get lower in both topologies.
In the complete topology, Europe and North America get slightly closer to the fair state, but there's still a large difference between them and other regions.

Based on the difference between Europe and North America with the remaining regions, we can explain the difference by the theoretical model mention above.
As large clusters with lower delay inside the cluster, they can get a higher accepted rate in their mined blocks, which corresponds to the two-cluster competition that the large cluster can gain more.
Since Europe has 94 nodes and North America has 83 nodes, they have 72\% of nodes in the network, which is also a good point to get the maximum percentiles on for every node.

\subsubsection{Artificial clustering into two clusters}
Natural clustering gives a great preference to the European and North American nodes.
Now we try some artificial clusterings to the whole network to learn the influence from the artificial topology.
We first implement the artificial clustering by randomly splitting the nodes into 70\% to simulate a large cluster and 30\% to simulate a small cluster.
Similar to the theoretical model, nodes are more likely to connect to the nodes in the same cluster and unlikely to connect to the nodes in the other cluster.
So we apply complete connections in each cluster but only leaves 20 connection between the 2 clusters.
 
\begin{figure*}[!tbp]
  \centering
  \subfigure[]{\includegraphics[width=0.5\textwidth]{Figures/random70Cluster.png}\label{fig:70cluster}}
~~
  \subfigure[]{\includegraphics[width=0.5\textwidth]{Figures/EuNACluster.png}\label{fig:EUNACluster}}
  \caption{TO DO.
  }
  \label{fig:ArtClustering}
\end{figure*}

Figure~\ref{fig:70cluster} shows that the nodes in the large cluster get more percentile of blocks with the help of the large cluster..
The European and North American nodes are even hard to reach the fair state if they are in the small cluster.

Then we try another topology that we take Europe and North America as the large cluster and the remaining continents as the small cluster.
With the same topology to have complete connections in each cluster and leave only 20 connects between clusters.
In Figure~\ref{fig:EUNACluster}, the percentile distributions are narrower compare with the random topology in Figure~\ref{fig:randomandcom}.
Cluster by the regions gives a more stable performance in each continent.


\subsubsection{How to alleviate bias due to clustering}
The 70\% clustering topology inspires the approach with artificial neighbor connections to alleviate the biases.
Thus we conduct experiments to adjust the neighbor degree.
We first focus the 




\begin{figure*}[!tbp]
  \centering
  \subfigure[]{\includegraphics[width=0.35\textwidth]{Figures/biasAtRemote.png}\label{fig:biasAtRemote}}
  \caption{TO DO.
  }
  \label{fig:biasAtRemote}
\end{figure*}

Figure show that Asian nodes can easily increase its percentile with more out-going neigh connections, while European nodes get less improvements and some nodes even decline from 24 to 48 neighbors.

\begin{figure*}[!tbp]
  \centering
  \subfigure[]{\includegraphics[width=0.35\textwidth]{Figures/biasAtRemote.png}\label{fig:biasAtEuNA}}
  \caption{TO DO.
  }
  \label{fig:biasAtEuNa}
\end{figure*}

Figure show that most European nodes get a less percentile after adding more neighbors, which is contradictory to the Asian nodes.
European and North American nodes have more advantage in the bitcoin mining competition than the other continents.
Thus we cluster those two continents nodes as central nodes while the others as remote nodes.
The central node cluster has more nodes and they are at the geographical central across the world, they have a shorter delay to all the others node so that they can broadcast their mined blocks quicker than the remote nodes.
During the time to broadcast their mined blocks, they can even mine the next block earlier, which can expand their advantage, so that we can see a significant difference between central nodes and remote nodes.

For the remote nodes, they need methods to increase their centrality to make up their disadvantage in cluster size and geographical distribution.
Perigee provides a way to learn the network efficiently so as to connect to more 'useful' neighbors.
Figure also shows that connecting more neighbor can do help increase the centrality, but maintaining more neighbor connections will aggravate the node processing time as it needs to exchange block information with all its neighbors.
So the ideal neighbor connection strategy for the remote node cluster is to learn the network, find the nodes with good connection to the network and connect to them as many as possible.

However, for the central nodes, there are 2 cases.
If there's only one central cluster, then it need to limit its connection as if it connects more neighbors, the remote node can get more advantage than the central nodes so the central node can only get some lost in the mining competition.
If there are multiple central cluster like European nodes and North American nodes. Connecting more neighbor can bring more advantage to the remote nodes but can also put pressure to the opposite central cluster. 
So the Ideal strategy is the trade-off between share advantage to the remote nodes and snatch profits from the opposite central cluster.

\begin{figure*}[!tbp]
  \centering
  \subfigure[]{\includegraphics[width=0.35\textwidth]{Figures/biasAtRemote.png}\label{fig:Perigee}}
  \caption{TO DO.
  }
  \label{fig:Perigee}
\end{figure*}


Perigee algorithm can efficiently decrease the broadcasting delay during message exchange.
A lower broadcasting delay correspond a higher mining time and a higher difficulty in the network.
A high difficulty network can provide a fairer state for the remote nodes, however the decrease in the broadcasting delay can only lead to a slightly relative change in the difficulty, so that the difference are not significant and most remote nodes can only occupy little percentile of valid blocks.
		
